Are Watermarked Images Editable? SafeMark for Watermark-Preserving Text-Guided Image Editing

This paper investigates a fundamental yet underexplored question: can watermarked images remain editable without compromising watermark integrity? We propose SafeMark, a framework for watermark-preserving text-guided image manipulation that explicitly integrates watermark integrity into the editing process. Specifically, SafeMark adds a thresholded watermark-decoding loss directly to the diffusion editor's training objective, fine-tuning the editor so that semantically valid edits also preserve the embedded watermark at the final output. This design admits a clean information-theoretic justification: maintaining high bit-accuracy on the edited image lower-bounds the mutual information that the editor channel preserves between watermark and edited output, the quantity that fundamentally controls watermark recoverability. SafeMark is compatible with differentiable diffusion-based editors, and requires no architectural modification. Extensive evaluations across multiple datasets, text-guided editing methods, and post-edit distortion settings demonstrate that SafeMark achieves high watermark bit accuracy across diverse editing settings while maintaining high-quality semantic edits, without sacrificing robustness to common post-edit distortions. These results demonstrate that semantic editability and watermark integrity are fundamentally compatible, enabling trustworthy image provenance in generative editing pipelines.

==> preamble.tex <==

\usepackage{xr-hyper}
\makeatletter
\newcommand*{\addFileDependency}[1]{\typeout{(#1)}\@addtofilelist{#1}\IfFileExists{#1}{}{\typeout{No file #1.}}}
\makeatother
\newcommand*{\myexternaldocument}[1]{\externaldocument[][nocite]{#1}\addFileDependency{#1.tex}\addFileDependency{#1.aux}}

\usepackage{currfile}
\usepackage{caption}
\usepackage[T1]{fontenc}
\usepackage{microtype}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{xspace}
\usepackage{xcolor}

\newcommand{\sysname}{SafeMark\xspace}
\newif\ifarxiv   %
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\makeatletter
\newbox\SM@labels
\let\SM@ShipoutPicture\@ShipoutPicture
\def\@ShipoutPicture{%
  \let\SM@inlabel\if@inlabel
  \global\setbox\SM@labels\box\@labels
  \global\@inlabelfalse
  \SM@ShipoutPicture
  \global\setbox\@labels\box\SM@labels
  \global\let\if@inlabel\SM@inlabel}
\makeatother

\AtBeginDocument{%
  \crefname{appendix}{Supp.~Sec.}{Supp.~Secs.}\Crefname{appendix}{Supplementary Section}{Supplementary Sections}%
  \crefname{subappendix}{Supp.~Sec.}{Supp.~Secs.}\Crefname{subappendix}{Supplementary Section}{Supplementary Sections}}

